Learning Pessimism for Robust and Efficient Off-Policy Reinforcement Learning

Off-policy deep reinforcement learning algorithms commonly compensate for overestimation bias during temporal-difference learning by utilizing pessimistic estimates of the expected target returns. In this work, we propose Generalized Pessimism Learning (GPL), a strategy employing a novel learnable penalty to enact such pessimism. In particular, we propose to learn this penalty alongside the critic with dual TD-learning, a new procedure to estimate and minimize the magnitude of the target returns bias with trivial computational cost. GPL enables us to accurately counteract overestimation bias throughout training without incurring the downsides of overly pessimistic targets. By integrating GPL with popular off-policy algorithms, we achieve state-of-the-art results in both competitive proprioceptive and pixel-based benchmarks.

==> Paper/Sections/OMITTEDAlgorithm.tex <==
\section{Algorithm implementation}
\label{sec:algs}
\begin{algorithm}[t]
    \caption{\textit{GPL-SAC}}
    \label{alg:GPLsac}
    \begin{algorithmic}[1]
    \Procedure{TrainingLoop}{$N, \textit{UTD}, \rho, \gamma, \hat{H}$}
    \State Initialize $\pi_\theta, \{Q_{\phi_i}^{\pi}\}^N_{i=1}, \{Q_{\phi'_i}^{\pi}\}^N_{i=1}, \beta\gets 0.5, \alpha\gets 0.0, D \gets \emptyset$
    \Loop
        \State Observe $s$ from the environment
        \State Execute $a\sim \pi_{\theta}(s)$ in the environment, collect $s', r$
        \State Store $D \gets D \cup (s, a, s', r)$
        \For{$j = 1, 2, ..., \textit{UTD}$}
        \State Sample minibatch $\{(s, a, s', r)\}\in D$
            \State Sample $a'\sim \pi(s')$
            %\State Approximate the \textit{uncertainty regularizer} and target action-values $$p_\beta(s', \phi', \theta) \gets \frac{\beta}{N^2-N}\sum_{i=1}^N \sum_{j\neq i}^N |Q_{\phi'_i}^{\pi}(s', a') - Q_{\phi'_j}^{\pi}(s', a')|, \bar{Q}_{\phi'}^\pi(s', a') \gets \frac{1}{N}\sum_{i=1}^N Q_{\phi'_i}^{\pi}(s', a')$$
            \State Compute $\hat{Q}_{\phi'}^\pi(s', a') \gets \textsc{RegularizedValue}(s', a', \phi', \theta, \beta)$
            \State Compute the TD-targets $y\gets r + \gamma\left(\hat{Q}_{\phi'}^\pi(s', a') - \alpha \log \pi(a'|s')\right)$
            \For{$i = 1, 2, ..., \textit{N}$}
                \State Compute the TD-errors for the $i^{th}$ critic $e_i\gets Q_{\phi_i}^{\pi} - y$
                \State Update ${\phi_i}$ to minimize $J(\phi)=e_i^2$ \Comment{Learning the critic}
                \State Update $\phi'_i\gets\rho\phi'_i + (1-\rho)\phi_i$ \Comment{Updating the target critic}
            \EndFor
            \EndFor
        \State Update ${\beta}$ to minimize $J(\beta) = \beta\times \sum_{i=1}^N e_i$ \Comment{Learning the bias (dual TD-learning)}
        \State Sample $a\sim \pi(s)$
        \State Compute $\hat{Q}_{\phi}^\pi(s, a) \gets \textsc{RegularizedValue}(s, a, \phi, \theta, \beta)$
        \State Update ${\theta}$ to minimize $J(\theta) = - \hat{Q}_{\phi_i}^{\pi}(s, a) + \alpha \log \pi(a|s)$ \Comment{Learning the policy}
        \State Update $\alpha$ to minimize $J(\alpha) = \alpha\times (- \log \pi(a|s) - \hat{H})$ \Comment{Learning the entropy bonus}
    \EndLoop
    \EndProcedure
    \Procedure{RegularizedValue}{$s, a, \phi, \theta, \beta$}
    \State Compute $p_\beta(s, \phi, \theta) \gets \frac{\beta}{N^2-N}\sum_{i=1}^N \sum_{j\neq i}^N |Q_{\phi_i}^{\pi}(s, a) - Q_{\phi_j}^{\pi}(s, a)|$ \State Compute $\bar{Q}_{\phi}^\pi(s, a) \gets \frac{1}{N}\sum_{i=1}^N Q_{\phi_i}^{\pi}(s, a)$
    \State \textbf{return} $\bar{Q}_{\phi}^\pi(s, a) - p_\beta(s, \phi, \theta)$
    \EndProcedure
    \end{algorithmic}
\end{algorithm}

% \begin{algorithm}
%     \caption{\textit{Routine off-policy framework}}
%     \label{routine_alg}
%     \begin{algorithmic}[1]
%     \State Initialize $\pi_\theta, Q_{\phi_1}^{\pi_\theta}, Q_{\phi_2}^{\pi_\theta}, D_{\omega_1}, E_{\omega_2}.$
%     \State Initialize $B_\pi \gets \emptyset$, $count\gets 0$
%     \For{$i = 1, 2, ...,$}
%         \State Observe $s$ from the environment
%         \State Query policy to obtain $n\sim \pi_{\theta}(s)$
%         \State Sample $a_1, a_2, ..., a_l \sim D_{\omega_1}(n)$
%         \For{$a = a_1, a_2, ..., a_l$}
%             \State Execute $a$ in the environment, collect $(s', r, t)$
%             \State Store $B = B \cup (s, a, s', r, t)$
%             \State Sample $b=\{(s, a_{1:L}, s_{1:L}', r_{1:L}, t_{1:L})_{|b|}\}\in B$
%             \For{$m = 1, 2$}
%                 \State Approximate $J_Q$ and $J_{lc}$ with $b$
%                 \State Update $Q^{\pi_\theta}_{\phi_m}$ with $\nabla_{\phi_m}J_Q$
%                 \State Update $D_{\omega_1}$, $E_{\omega_2}$ with $\nabla_{\omega}(J_Q+J_{lc})$
%             \EndFor
%             \State Update $count\gets count + 1$
%             \IF{$count \mod delay$ = 0}
%                 \State Approximate $J_\pi$ and $J_{mto}$ with $b$
%                 \State Update $\pi_\theta$ with $\nabla_{\theta}J_\pi$
%                 \State Update $D_{\omega_1}$ with $\nabla_{\omega_1}(J_\pi-J_{mto})$
%             \ENDIF
%         \EndFor
%     \EndFor
%     \end{algorithmic}
% \end{algorithm}

We integrate \textit{GPL} to extend two state-of-the-art off-policy RL algorithms and describe the main effective difference below. We further provide a list of the utilized hyper-parameters in Section \edo{app} of the Appendix. We open-source our code to facilitate future comparisons and extensions.

\subsection{Integration with soft actor-critic}

For testing \textit{GPL} for control problems from proprioceptive states, we integrate our  procedure, as described in Section~\ref{sec:method}, with \textit{Soft Actor-Critic (SAC)} \citep{sac, sac-alg}, a popular model-free off-policy algorithms that uses a weighted entropy term in its objective to incentivize exploration. For counteracting the overestimation bias, we substitute \textit{SAC}'s \textit{clipped double Q-learning} procedure with the proposed \textit{uncertainty regularizer}, initialized with $\beta=0.5$. We also adopt several other algorithmic changes inspired by related recent successes \citep{mbpo, redq, deeper-deep-RL}. Particularly, we parameterize ten independent action-value functions, $\{Q^\pi_{\phi_i}\}^N_{i=1}$, and increase the update-to-data ratio (UTD) for the action-value function to twenty. Moreover, we represent each critic as a simple two-layers residual neural networks with spectral normalization applied to only the hidden layer \citep{sngan}. We initialize $\beta = 0.5$, such that the initial penalty has the same expected scale as \textit{clipped double Q-learning}, yet computed by using all ten critics. We denote the resulting algorithm \textit{GPL-SAC} and provide a schematic summary of this integration in Algorithm~\ref{alg:GPLsac}. % and \citep{}, such as increasing the number of critics from the 

\subsection{Integration with drq-v2}

We also integrate \textit{GPL} with the recent \textit{DrQ-v2} algorithm \citep{drqv2} for pixel-based control problems. \textit{DrQ-v2} combines the image augmentation strategy from \textit{DrQ} \citep{drq} with several advances such as n-step returns \citep{sutton-reinforcement-n-step} and scheduled exploration noise \citep{scheduled-exploration-noise}. Again, we substitute \textit{DrQ-v2}'s\textit{clipped double Q-learning} procedure with the proposed \textit{uncertainty regularizer} initialized with $\beta=0.5$. we also make use of the \textit{optimistic shifted uncertainty regularizer} described in Section~\ref{sec:act-shift}, with $\lambda_{opt}$ linearly decayed from 0.5 to 0.0, together with the exploration noise in \textit{DrQ-v2}. This procedure should be particularly effective in pixel-based environments which tend to involve inherently harder exploration challenges from the high dimensionality of their state-space. We leave the rest of the original hyper-parameters and model architectures unaltered to specifically analyze the generality of applying \textit{GPL}. We denote the resulting algorithm \textit{GPL-DrQ}. %and \textit{GPL-DrQ-Expl+}, respectively.

\subsection{Implementation considerations}

In both implementations, \textit{GPL} introduces trivial computational costs as it optimizes a single weight by re-utilizing the computed errors in the TD-loss to estimate the bias. Moreover, in contrast with many prior implementations of model-free off-policy algorithms, we implement the ensemble of action-value models as a single neural network making use of linear non-fully-connected layers, evenly splitting the nodes and dropping the weight connections between the splits. Practically, when evaluated under the same hardware, this results in our algorithm running more than three times faster than the implementation from \citet{redq}, while having a similar algorithmic complexity. %prior work with a similar algorithmic complexity \citep{redq}. 
For further details, please refer to our open-source implementation.

% \subsection{Enforcing the mutual information constraints}
% \label{mi-const-enf}

% We implement two different techniques to enforce the mutual information constraints proposed in Section~\ref{mireg}, given a set of observations $B$ with the corresponding domain labels. Both techniques make use of a single hyper-parameter $I_{max}$, which represents the upper limit on the estimated information about the domain labels that we allow the latent representations to retain.

% \textbf{Adaptive penalty $L_\beta$}. The first technique is having a supplementary loss function for the preprocessor $P_{\theta_1}$, penalizing it proportionally to the estimated mutual information in the latent representations. We use an adaptive parameter $\beta$ to ensure the mutual information is within the desired range:
% \begin{equation}
% \label{beta-pen}
% L_\beta(\theta_1, B)=\beta I_\phi(\mathbf{z}_i, d_i|B).
% \end{equation}
% We design our updates of $\beta$ to follow a similar pattern to the adaptive penalty coefficient proposed by \citet{ppo}, utilizing $I_{max}$ and updating:
% \begin{tasks}[style=itemize](2)
% \task $\beta \leftarrow \beta\times 1.5$, \textit{if} $I_\phi(\mathbf{z}_i, d_i|B) > I_{max}$
% \task $\beta \leftarrow \beta\div 1.5$, \textit{if} $I_\phi(\mathbf{z}_i, d_i|B) < I_{max}\div 2.$
% \end{tasks}
% \textbf{Dual penalty $L_\lambda$}. The second technique consists in a different supplementary loss function penalizing the preprocessor $P_{\theta_1}$ proportionally to the violation of the upper limit. In this case, we ensure constraint enforcement through the introduction of a non-negative Lagrange multiplier variable $\lambda$:
% \begin{equation}
% \label{lambda-pen}
% L_\lambda(\theta_1, B)=\lambda \left(I_\phi\left(\mathbf{z}_i, d_i|B\right) - I_{max}\right)
% \end{equation}
% where $\lambda$ is updated to maximize $L_\lambda$, approximating dual gradient descent \citep{convex}: 
% \begin{equation}
% \lambda \leftarrow \max\left(0, \lambda +  \alpha\left(I_\phi\left(\mathbf{z}_i, d_i|B\right) - I_{max}\right)\right).
% \end{equation}
 
% In practice, the dual penalty enforces precisely the mutual information constraints, but the dual variable $\lambda$ stabilizes in more iterations than the adaptive parameter $\beta$.
% Our final implementation makes use of the adaptive penalty when enforcing the expert demonstrations constraint with $I_{max}=0.99$ and the dual penalty when enforcing the prior data constraint with $I_{max}=0.001$. Hence, our penalized discriminator objective augments the original discriminator objective in Eq.~\ref{gail-obj} as:
% \begin{equation}
% \label{D-obj}
% \argmax_\theta J_G(\theta, B_E \cup B_\pi) - L_\beta(\theta_1, B_E \cup B_\pi) - L_\lambda(\theta_1, B_{P.E} \cup B_{P.\pi}).
% \end{equation}
% \subsection{Domain information disguising}

% \label{mi-fooling}
% The discriminator $D_\theta$ is updated to maximize Eq.~\ref{D-obj}, given a mutual information estimate from a fixed-sized statistics network $T_\phi$. Hence, if the optimization of $T_\phi$ temporarily converges to a sub-optimal local minimum, $D_\theta$ could encode domain information into the latent representations $\mathbf{z}$ without the statistics network detecting it. We refer to this phenomenon as \emph{domain information disguising}, and we utilize two further techniques to prevent this issue. 

% \textbf{Double statistics network}. The first technique takes inspiration from the work of \citet{double-q} and consists of learning independently two statistics neural networks, namely $T_{\phi_1}$ and $T_{\phi_2}$. Thus, the mutual information is estimated through taking the maximum prediction of the independent models over the same set of observations,  $\hat{I}_\phi(\mathbf{z}_i, d_i|B) = \max(I_{\phi_1}(\mathbf{z}_i, d_i|B), I_{\phi_2}(\mathbf{z}_i, d_i|B)).$ This change makes it impractical for the discriminator to disguise domain information, as the gradient from each of the regularization losses can only contain information about a single statistics network at a time (from the $\max$ operation). Therefore, this gives a statistics network reaching a sub-optimal local minimum the chance to recover, without affecting the mutual information estimates to a great extent. This practice has also the benefit of providing a better prediction of the current mutual information, counteracting the effects of epistemic uncertainty on the optimization.

% \textbf{Invariant discriminator regularization}. The second technique comprises regularizing the invariant discriminator $S_{\theta_2}$ to be approximately 1-Lipschitz. A great part of the GAN literature \citep{wass, wass-gp, sngan} showed the effectiveness of this practice when regularizing discriminator networks. In our specific problem setting, it has the further benefit of restricting the expressivity of the invariant discriminator, preventing it from capturing domain information not captured by our mutual information estimator. To enforce this, we utilize spectral normalization, a regularization technique proposed by~\citet{sngan}.


% \textit{DisentanGAIL} trains all the models end-to-end, in three main learning steps:
% (i) \textit{Discriminator learning}, where the discriminator's parameters $\theta$ are updated to maximize Eq.~\ref{D-obj}; (ii) \textit{Mutual information learning}, where the statistics network's parameters $\phi$ are updated to maximize Eq.~\ref{mi-opt}; (iii) \textit{Agent learning}, where the learner's parameters $\omega$ are updated to maximize Eq.~\ref{pi-opt} with SAC.
% We provide further implementation details and a formal summary of the algorithm in  Appendix~\ref{app:params}. 


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

